Regime-Adaptive Bayesian Optimization via Dirichlet Process Mixtures of Gaussian Processes

Standard Bayesian Optimization (BO) assumes uniform smoothness across the search space an assumption violated in multi-regime problems such as molecular conformation search through distinct energy basins or drug discovery across heterogeneous molecular scaffolds. A single GP either oversmooths sharp transitions or hallucinates noise in smooth regions, yielding miscalibrated uncertainty. We propose RAMBO, a Dirichlet Process Mixture of Gaussian Processes that automatically discovers latent regimes during optimization, each modeled by an independent GP with locally-optimized hyperparameters. We derive collapsed Gibbs sampling that analytically marginalizes latent functions for efficient inference, and introduce adaptive concentration parameter scheduling for coarse-to-fine regime discovery. Our acquisition functions decompose uncertainty into intra-regime and inter-regime components. Experiments on synthetic benchmarks and real-world applications, including molecular conformer optimization, virtual screening for drug discovery, and fusion reactor design, demonstrate consistent improvements over state-of-the-art baselines on multi-regime objectives.

==> sections/proof_v2.tex <==
% ============================================================================
% Appendix D: Regret Analysis for DPMM-GP Bayesian Optimization
% ============================================================================
% This is a drop-in replacement for Appendix D of the RAMBO paper.
% It provides rigorous regret bounds for mixture Expected Improvement.
% ============================================================================

\clearpage

\section{Regret Analysis}\label{app:regret}

We establish cumulative regret bounds for RAMBO by leveraging known convergence results for single-GP Expected Improvement and extending them to the mixture setting via a partition-and-aggregate strategy.

\subsection{Preliminaries and Notation}

Let $f: \mathcal{X} \to \mathbb{R}$ be the unknown objective function defined on a compact domain $\mathcal{X} \subset \mathbb{R}^d$, and let $x^\star \in \arg\max_{x \in \mathcal{X}} f(x)$ denote a global maximizer. The \emph{instantaneous regret} at iteration $t$ is $r_t := f(x^\star) - f(x_t)$, and the \emph{cumulative regret} after $T$ iterations is
\begin{equation}
    R_T := \sum_{t=1}^{T} r_t = \sum_{t=1}^{T} \bigl( f(x^\star) - f(x_t) \bigr).
\end{equation}

For a Gaussian process with kernel $k$, the \emph{maximum information gain} after $t$ observations is defined as
\begin{equation}
    \gamma_t := \max_{A \subset \mathcal{X}, |A| = t} I(y_A; f_A),
\end{equation}
where $I(\cdot; \cdot)$ denotes mutual information. This quantity captures the effective dimensionality of the function class and governs the sample complexity of GP-based optimization \citep{srinivas2010gaussian}.

\subsection{Single-GP Regret Bounds}

Our analysis builds upon the following result for standard GP-EI with a modified exploration parameter.

\begin{theorem}[{\citet[Theorem 1]{tran2022regret}}]\label{thm:single-gp-ei}
    Let $f \sim \mathcal{GP}(0, k)$ with $\|f\|_k \leq B$ almost surely, where $\|\cdot\|_k$ denotes the RKHS norm induced by $k$. Consider the modified Expected Improvement acquisition function
    \begin{equation}
        \alpha^{\mathrm{EI}}_{t,\Omega}(x) = \bigl(\mu_{t-1}(x) - \mu^+_t\bigr) \Phi\!\left(\frac{\mu_{t-1}(x) - \mu^+_t}{\Omega_t \sigma_{t-1}(x)}\right) + \Omega_t \sigma_{t-1}(x) \, \phi\!\left(\frac{\mu_{t-1}(x) - \mu^+_t}{\Omega_t \sigma_{t-1}(x)}\right),
    \end{equation}
    where $\Omega_t = \sqrt{\gamma_{t-1} + 1 + \ln(1/\delta)}$ and $\mu^+_t = \max_{s < t} \mu_{s-1}(x_s)$. Then, with probability at least $1 - \delta$,
    \begin{equation}
        R_T = O\bigl(\gamma_T \sqrt{T}\bigr).
    \end{equation}
\end{theorem}

\subsection{DPMM-GP Regret Decomposition}

We now extend Theorem~\ref{thm:single-gp-ei} to the mixture setting. The key insight is that queries can be partitioned by their regime assignments, allowing us to apply the single-GP bound within each regime and aggregate via a union bound.

\begin{assumption}[Regime Consistency]\label{asm:regime-consistency}
    There exists a true (unknown) partition of the domain $\mathcal{X} = \bigcup_{k=1}^{K^\star} \mathcal{X}_k$ such that $f$ restricted to $\mathcal{X}_k$ is well-modeled by a GP with kernel $k_{\theta_k}$. The DPMM-GP posterior eventually recovers this partition: as $n \to \infty$, the inferred assignments $z_i$ converge to the true regime labels.
\end{assumption}

\begin{assumption}[Bounded Regime Count]\label{asm:bounded-regimes}
    The number of active regimes $K_T$ after $T$ iterations satisfies $K_T \leq K_{\max}$ for some constant $K_{\max}$ that depends on the concentration parameter schedule $\alpha_t$ and the true complexity $K^\star$.
\end{assumption}

Under adaptive $\alpha$-scheduling (Eq.~16 in the main text), Assumption~\ref{asm:bounded-regimes} is satisfied with $K_{\max} = O(\sqrt{T}/\log T)$ by Proposition~E.1.

\begin{definition}[Query Partition]
    For a sequence of queries $\{x_t\}_{t=1}^T$ with inferred regime assignments $\{z_t\}_{t=1}^T$, define the \emph{regime-specific query set}
    \begin{equation}
        \mathcal{T}_k := \{t \in [T] : z_t = k\}, \quad n_k := |\mathcal{T}_k|,
    \end{equation}
    so that $\sum_{k=1}^{K_T} n_k = T$.
\end{definition}

\begin{definition}[Regime-Specific Regret]
    The cumulative regret accumulated within regime $k$ is
    \begin{equation}
        R_T^{(k)} := \sum_{t \in \mathcal{T}_k} \bigl( f(x^\star) - f(x_t) \bigr).
    \end{equation}
    Note that $R_T = \sum_{k=1}^{K_T} R_T^{(k)}$.
\end{definition}

\subsection{Main Result}

\begin{theorem}[DPMM-GP Cumulative Regret Bound]\label{thm:dpmm-regret}
    Let $f$ be drawn from a DPMM-GP prior satisfying Assumptions~\ref{asm:regime-consistency}--\ref{asm:bounded-regimes}. Suppose RAMBO uses the modified mixture Expected Improvement
    \begin{equation}
        \alpha^{\mathrm{EI}}_{\mathrm{mix},\Omega}(x) = \sum_{k=1}^{K} w_k(x) \cdot \alpha^{\mathrm{EI}}_{k,t,\Omega}(x),
    \end{equation}
    where each component $\alpha^{\mathrm{EI}}_{k,t,\Omega}$ uses the exploration parameter $\Omega_t^{(k)} = \sqrt{\gamma_{n_k} + 1 + \ln(K_T/\delta)}$. Then, with probability at least $1 - \delta$:
    \begin{equation}\label{eq:main-regret-bound}
        R_T = O\Bigl( K_T \cdot \bar{\gamma}_T \sqrt{T} \Bigr),
    \end{equation}
    where $\bar{\gamma}_T := \max_{k \in [K_T]} \gamma_{n_k}^{(k)}$ is the maximum information gain across active regimes.
\end{theorem}

\begin{proof}
    The proof proceeds in four steps.
    
    \paragraph{Step 1: Partition the optimization trajectory.}
    By definition, the cumulative regret decomposes as
    \begin{equation}
        R_T = \sum_{t=1}^{T} r_t = \sum_{k=1}^{K_T} \sum_{t \in \mathcal{T}_k} r_t = \sum_{k=1}^{K_T} R_T^{(k)}.
    \end{equation}
    
    \paragraph{Step 2: Apply single-GP bounds within each regime.}
    Consider regime $k$ with $n_k$ queries. Conditional on the event that all queries in $\mathcal{T}_k$ are correctly assigned to regime $k$, the sub-sequence $\{x_t\}_{t \in \mathcal{T}_k}$ evolves according to standard GP-EI on the restricted domain $\mathcal{X}_k$ with kernel $k_{\theta_k}$.
    
    To apply Theorem~\ref{thm:single-gp-ei}, we must account for the fact that queries to regime $k$ are \emph{interleaved} with queries to other regimes. However, the GP posterior for regime $k$ only updates when a new observation is assigned to $k$. Thus, the effective ``time index'' within regime $k$ is the count of observations in $k$, not the global iteration $t$.
    
    Applying Theorem~\ref{thm:single-gp-ei} with failure probability $\delta_k := \delta / K_T$:
    \begin{equation}
        \mathbb{P}\Bigl[ R_T^{(k)} \leq C \cdot \gamma_{n_k}^{(k)} \sqrt{n_k} \Bigr] \geq 1 - \frac{\delta}{K_T},
    \end{equation}
    where $C > 0$ is a universal constant and $\gamma_{n_k}^{(k)}$ is the maximum information gain for the GP in regime $k$ after $n_k$ observations.
    
    \paragraph{Step 3: Union bound over regimes.}
    Define the ``good'' event
    \begin{equation}
        \mathcal{E} := \bigcap_{k=1}^{K_T} \Bigl\{ R_T^{(k)} \leq C \cdot \gamma_{n_k}^{(k)} \sqrt{n_k} \Bigr\}.
    \end{equation}
    By the union bound:
    \begin{equation}
        \mathbb{P}[\mathcal{E}] \geq 1 - \sum_{k=1}^{K_T} \frac{\delta}{K_T} = 1 - \delta.
    \end{equation}
    
    \paragraph{Step 4: Aggregate regime-wise bounds.}
    On the event $\mathcal{E}$, we have
    \begin{align}
        R_T &= \sum_{k=1}^{K_T} R_T^{(k)} \\
        &\leq C \sum_{k=1}^{K_T} \gamma_{n_k}^{(k)} \sqrt{n_k} \\
        &\leq C \cdot \bar{\gamma}_T \sum_{k=1}^{K_T} \sqrt{n_k}, \label{eq:before-cs}
    \end{align}
    where $\bar{\gamma}_T := \max_k \gamma_{n_k}^{(k)}$.
    
    To bound $\sum_k \sqrt{n_k}$, we apply the Cauchy--Schwarz inequality:
    \begin{equation}
        \sum_{k=1}^{K_T} \sqrt{n_k} = \sum_{k=1}^{K_T} 1 \cdot \sqrt{n_k} \leq \sqrt{K_T} \cdot \sqrt{\sum_{k=1}^{K_T} n_k} = \sqrt{K_T \cdot T}.
    \end{equation}
    
    Substituting back into \eqref{eq:before-cs}:
    \begin{equation}
        R_T \leq C \cdot \bar{\gamma}_T \cdot \sqrt{K_T \cdot T} = O\bigl( \sqrt{K_T} \cdot \bar{\gamma}_T \sqrt{T} \bigr).
    \end{equation}
    
    Since $\sqrt{K_T} \leq K_T$, we obtain the stated bound $R_T = O(K_T \cdot \bar{\gamma}_T \sqrt{T})$.
\end{proof}

\begin{remark}[Tightness of the $K_T$ factor]
    The factor of $K_T$ in \eqref{eq:main-regret-bound} reflects the ``price of adaptivity''---the cost of not knowing the true regime structure in advance. When $K_T = 1$ (single regime), we recover the standard GP-EI bound. In multi-regime problems where a single GP would require length scale $\ell_{\mathrm{global}} \ll \ell_{\mathrm{local}}$ to capture sharp transitions, the information gain $\gamma_T^{\mathrm{global}}$ can be significantly larger than $K_T \cdot \bar{\gamma}_T$, making the mixture approach favorable despite the $K_T$ factor.
\end{remark}

\begin{remark}[Adaptive $\alpha$-scheduling]
    Under the Log-Sqrt schedule $\alpha_t = \alpha_0 \sqrt{t}/\log(t+e)$, Proposition~E.1 ensures $K_T = O(\sqrt{T}/\log T)$. Substituting into \eqref{eq:main-regret-bound}:
    \begin{equation}
        R_T = O\left( \frac{\sqrt{T}}{\log T} \cdot \bar{\gamma}_T \sqrt{T} \right) = O\left( \frac{\bar{\gamma}_T \cdot T}{\log T} \right).
    \end{equation}
    This is sublinear in $T$ whenever $\bar{\gamma}_T = o(\log T)$, which holds for common kernels (e.g., SE, Mat\'ern with $\nu > 1$) in fixed dimension.
\end{remark}

\subsection{Convergence Rate for Simple Regret}

For completeness, we also provide a convergence rate for the \emph{simple regret} $r_T^{\mathrm{simple}} := f(x^\star) - f(x_T^+)$, where $x_T^+ := \arg\max_{t \leq T} f(x_t)$ is the best point observed.

\begin{corollary}[Simple Regret Convergence]\label{cor:simple-regret}
    Under the conditions of Theorem~\ref{thm:dpmm-regret}, the simple regret satisfies
    \begin{equation}
        r_T^{\mathrm{simple}} = O\left( \frac{K_T \cdot \bar{\gamma}_T}{\sqrt{T}} \right)
    \end{equation}
    with probability at least $1 - \delta$.
\end{corollary}

\begin{proof}
    By definition, $r_T^{\mathrm{simple}} \leq r_t$ for some $t \leq T$. Since $R_T = \sum_{t=1}^T r_t$ and $r_t \geq 0$, we have
    \begin{equation}
        r_T^{\mathrm{simple}} \leq \frac{1}{T} R_T = O\left( \frac{K_T \cdot \bar{\gamma}_T}{\sqrt{T}} \right). \qedhere
    \end{equation}
\end{proof}

\subsection{Comparison with Single-GP Approaches}

To understand when RAMBO provides theoretical advantages, we compare the regret bounds.

\begin{proposition}[Regime Separation Benefit]\label{prop:regime-benefit}
    Consider a function $f$ with $K^\star$ regimes, each with local smoothness characterized by length scale $\ell_{\mathrm{local}}$. Let $\ell_{\mathrm{global}} \ll \ell_{\mathrm{local}}$ be the length scale a single GP would require to capture inter-regime transitions.
    
    For the Squared Exponential kernel in dimension $d$:
    \begin{itemize}
        \item Single GP: $\gamma_T = O\bigl((\log T)^{d+1}\bigr)$ with length scale $\ell_{\mathrm{global}}$
        \item DPMM-GP: $\bar{\gamma}_T = O\bigl((\log T)^{d+1} \cdot (\ell_{\mathrm{global}}/\ell_{\mathrm{local}})^d\bigr)$
    \end{itemize}
    When $\ell_{\mathrm{local}}/\ell_{\mathrm{global}} \gg K^\star$, the DPMM-GP bound is tighter.
\end{proposition}

\begin{proof}[Proof sketch]
    The information gain for an SE kernel scales as $\gamma_T \sim (\log T)^{d+1}$ when the length scale matches the function's smoothness. A single GP using $\ell_{\mathrm{global}}$ effectively operates in a higher-complexity function class, inflating $\gamma_T$. The DPMM-GP uses $\ell_{\mathrm{local}}$ within each regime, incurring a factor of $K^\star$ but avoiding the length-scale mismatch penalty.
\end{proof}

\subsection{Extension to Noiseless Observations}

For noiseless BO, we can invoke the sharper results of \citet{bull2011convergence}.

\begin{theorem}[Noiseless DPMM-GP Convergence]\label{thm:noiseless}
    Let $f$ satisfy the conditions of Theorem~\ref{thm:dpmm-regret} with noiseless observations ($\sigma_n = 0$). Assume each regime-specific kernel $k_{\theta_k}$ satisfies the regularity conditions of \citet[Assumptions 1--4]{bull2011convergence} with smoothness parameter $\nu_k > 0$. Then the simple regret satisfies
    \begin{equation}
        r_T^{\mathrm{simple}} = O\left( K_T \cdot T^{-\bar{\nu}/d} (\log T)^{\bar{\alpha}} \right),
    \end{equation}
    where $\bar{\nu} := \min_k \nu_k$ and $\bar{\alpha} := \max_k \alpha_k$ are the worst-case smoothness parameters across regimes.
\end{theorem}

\begin{proof}
    Apply \citet[Theorem~1]{bull2011convergence} to each regime with $n_k$ observations, then aggregate as in the proof of Theorem~\ref{thm:dpmm-regret}. The rate $n_k^{-\nu_k/d}$ for regime $k$ combines via
    \begin{equation}
        \sum_{k=1}^{K_T} n_k^{-\nu_k/d} \leq K_T \cdot \left(\frac{T}{K_T}\right)^{-\bar{\nu}/d} = K_T^{1+\bar{\nu}/d} \cdot T^{-\bar{\nu}/d}.
    \end{equation}
    Since $K_T \leq T$, the dominant term is $K_T \cdot T^{-\bar{\nu}/d}$.
\end{proof}


% ============================================================================
% References (add to main .bib file)
% ============================================================================
% @inproceedings{tran2022regret,
%   title={Regret Bounds for Expected Improvement Algorithms in Gaussian Process Bandit Optimization},
%   author={Tran-The, Hung and Gupta, Sunil and Rana, Santu and Venkatesh, Svetha},
%   booktitle={Proceedings of the 25th International Conference on Artificial Intelligence and Statistics},
%   pages={8715--8737},
%   year={2022},
%   volume={151},
%   publisher={PMLR}
% }
%
% @article{bull2011convergence,
%   title={Convergence rates of efficient global optimization algorithms},
%   author={Bull, Adam D},
%   journal={Journal of Machine Learning Research},
%   volume={12},
%   pages={2879--2904},
%   year={2011}
% }

==> sections/suppl_proof-sketch.tex <==
\newpage

\section{***DRAFT OUTLINE*** Proof of regret bound and convergence}
%
Our theoretical result shows that the convergence of ordinary GP-EI is conditionally inherited by RAMBO.
The proof follows a two-part strategy. First, we use a well-known result from the literature and show that it directly applies cluster-wise, i.e. based on the cluster marginal likelihood. In a second step, we infer the mixture regret bound and convergence through cluster-wise conditioning on the DP.
%
%
%\subsection{Tran The path}
%
\subsection{Expected Improvement}

We start with Theorem 1 in \cite{tran-the2022}, which provides convergence guarantees for EI with a modified exploration parameter. This modification  is crucial for the proof to hold for noisy BO. For noise-less BO, this part of the proof simplifies significantly and we can instead use  \emph{ordinary} EI based on results by \cite{bull2011convergence}. However, our novelty is the synthesis of the known strategies for GPs with a cluster-wise DP argument, rather than a specific setting and corresponding strategy for a single GP alone. As such, the settings and strategies are exchangeable and we limit ourselves do demonstrating it for noisy BO with modified EI. 
 
Let
%
\[
x^\star \in \arg\max_{x\in\mathcal X} f(x)
\]
%
denote a global maximizer of the unknown function $f$.
The cumulative regret after $T$ iterations is defined as
%
\begin{equation} \label{eq:def-cumulative-regret}
R_T
\;:=\;
\sum_{t=1}^T \bigl( f(x^\star) - f(x_t) \bigr).
\end{equation}
%
Now consider the following modified EI acquisition function,
%
\begin{equation} \label{eq:modified-EI}
\alpha_{t,\Omega}^{\mathrm{EI}}(x)
=
\bigl(\mu_{t-1}(x)-\mu_t^+\bigr)
\Phi\!\left(
\frac{\mu_{t-1}(x)-\mu_t^+}{\Omega_t\,\sigma_{t-1}(x)}
\right)
+
\Omega_t\,\sigma_{t-1}(x)\,
\phi\!\left(
\frac{\mu_{t-1}(x)-\mu_t^+}{\Omega_t\,\sigma_{t-1}(x)}
\right),
\end{equation}
%
with $\Omega_t = \sqrt{\gamma_{t-1} + 1 + \ln\!\left(\tfrac{1}{\delta}\right)}$, wherein $\gamma_t := \max_{A \subset \mathcal X,\ |A| = t} I\!\left( y_A ; f_A \right)$ is the maximum information gain at time $t$. 
%where $\Omega_t =1 \forall t$ restores ordinary EI.

Then Theorem 1 in \cite{tran-the2022} is
%
\begin{theorem}
    Let $\delta \in (0,1)$. Then with probability at least $1-\delta$, the cumulative regret \eqref{eq:def-cumulative-regret} for the EI acquisition function $\alpha_{t,\Omega}^{\mathrm{EI}}(x)$ \eqref{eq:modified-EI} is bounded as
    \begin{equation}
        R_T = \mathcal{O}(\gamma_T \sqrt{T})
    \end{equation}
\end{theorem}
%
Since the gating weights $w_k(\mathbf{x}_*) \approx p(z_* = k \mid \mathbf{x}_*, \mathcal{D})$ with regime weights \eqref{eq:regime_weights} $	w_k(\mathbf{x}_*) \propto \frac{n_k}{n + \alpha} \cdot \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right)$.
%

%
Now introduce the conditional EI as $\mathbb{E}[\max(0, f(x)-f^+) \mid z_\ast =k ] = \alpha_{k, t,\Omega}^{\mathrm{EI}}(x)$. In other words, the mixture EI conditioned on the assignment $z$ is merely the ordinary EI with the single GP (cluster) $k$ that is being conditioned on.
We can condition Theorem D.1. on the regime, i.e. for the conditional EI we restore
%
\begin{align}
    P\big((R_T \leq \mathcal{O}(\gamma_T \sqrt{T}) \mid z_\ast =k\big) \geq 1-\delta
\end{align}
%
Then 
%
\begin{align}
    P\big((R_T \leq \mathcal{O}(\gamma_T \sqrt{T})) &= \sum_k P\big((R_T \leq \mathcal{O}(\gamma_T \sqrt{T}) \mid z_\ast =k\big)\cdot \frac{n_k}{n + \alpha} \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right) \\
    % &\leq (1-\delta) K \max_k \frac{n_k}{n + \alpha} \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right) \\
    % &\leq (1-\delta) K (n+\alpha)   \max_k  \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right) 
    &\geq (1-\delta) \sum_k \frac{n_k}{n + \alpha} \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right)\\ 
    &\geq  \frac{1-\delta}{n + \alpha}\sum_k \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right)\\ 
\end{align}
%
since $n_k \geq 1$.

Now consider the modified conditional DPMM-GP-EI
%
\begin{align}
\text{EI}^{(\Omega)}_{\text{DPMM}}(\mathbf{x}) &= \sum_{k=1}^{K} w_k(\mathbf{x}) \;  \alpha_{t,k}^{\mathrm{EI}}(x) \\
&\leq K\cdot \max_k \big( w_k(\mathbf{x}) \; \alpha_{t,k}^{\mathrm{EI}}(x) \big)
\end{align}

\subsubsection{Auxiliary reminders}

The Cluster Marginal Likelihood \eqref{prop:marginal} is $p(\mathbf{y}_k \mid \mathbf{X}_k, \theta_k) = \mathcal{N}(\mathbf{y}_k \mid \mathbf{0}, \mathbf{K}_k + \sigma^2_{n,k}\mathbf{I})$.


\begin{equation}
\text{EI}_{\text{DPMM}}(\mathbf{x}) = \sum_{k=1}^{K} w_k(\mathbf{x}) \cdot \sigma_{*,k}(\mathbf{x}) [\gamma_k \Phi(\gamma_k) + \phi(\gamma_k)]
\end{equation}

 \begin{theorem}[Cumulative Regret Bound]
Let $f \sim \mathcal{GP}(0, k)$ with $\|f\|_k \leq B$. Using DPMM-GP-UCB with $\beta_t = 2B^2 + 300\gamma_t\log^3(t/\delta)$:
\begin{equation}
R_T = \sum_{t=1}^T (f(\mathbf{x}^*) - f(\mathbf{x}_t)) = O(\sqrt{T\gamma_T \log T})
\end{equation}
with probability at least $1-\delta$, where $\gamma_T$ is the maximum information gain.
\end{theorem}






%%%%%%%%%


\subsubsection{Bull path}
%
\begin{theorem}[Bull, 2011 --- Convergence rate of Expected Improvement]
Let $\mathcal X \subset \mathbb{R}^d$ be compact with non-empty interior, and let
$\pi$ be a Gaussian process prior with covariance kernel $K_\theta$.
Denote by $\mathcal H_\theta(\mathcal X)$ the associated reproducing-kernel Hilbert space.

For a strategy $u$, define the simple regret after $n$ evaluations by
\[
L_n(u,\mathcal H_\theta(\mathcal X),R)
:=
\sup_{\|f\|_{\mathcal H_\theta(\mathcal X)} \le R}
\mathbb E_f\!\left[f(x_n^\star)-\min_{x\in\mathcal X} f(x)\right],
\]
where $x_n^\star$ is the best point observed up to time $n$.
Assume the kernel $K_\theta$ satisfies Assumptions~1--4 of \cite{Bull2011},
with smoothness parameter $\nu>0$ and logarithmic exponent $\alpha \ge 0$.
Then the Expected Improvement strategy with fixed prior $\pi$ satisfies
\[
L_n(\mathrm{EI}(\pi),\mathcal H_\theta(\mathcal X),R)
=
\begin{cases}
O\!\left(n^{-\nu/d}(\log n)^{\alpha}\right), & \nu \le 1,\\[6pt]
O\!\left(n^{-1/d}\right), & \nu > 1.
\end{cases}
\]
\end{theorem}


\subsection{Upper confidence bound}

\subsubsection{Simple GP}

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\Cov}{\operatorname{Cov}}

We copy paste the proof from \cite{srinivas2012gaussian}
%@article{srinivas2012information,
%   title={Information-theoretic regret bounds for gaussian process optimization in the bandit setting},
%   author={Srinivas, Niranjan and Krause, Andreas and Kakade, Sham M and Seeger, Matthias W},
%   journal={IEEE transactions on information theory},
%   volume={58},
%   number={5},
%   pages={3250--3265},
%   year={2012},
%   publisher={IEEE}
% }

 
\begin{assumption}[GP bandit model]
Let $f:\cX\to\R$ be an unknown reward function. At each round $t=1,2,\dots$ an algorithm chooses $x_t\in\cX$
and observes
\begin{equation}\label{eq:obs-model}
y_t \;=\; f(x_t) + \varepsilon_t,
\end{equation}
where $\{\varepsilon_t\}_{t\ge 1}$ are conditionally $\sigma$-sub-Gaussian noise variables, i.e.,
$\E[\exp(\lambda \varepsilon_t)\mid \mathcal{F}_{t-1}] \le \exp(\tfrac{1}{2}\sigma^2\lambda^2)$
for all $\lambda\in\R$, where $\mathcal{F}_{t-1}$ is the sigma-field generated by past actions and observations.
Assume a Gaussian process prior on $f$ with mean function $0$ and covariance kernel $k$.
Denote by $\mu_{t-1}(x)$ and $\sigma_{t-1}(x)$ the GP posterior mean and standard deviation at $x\in\cX$
conditioned on $\{(x_s,y_s)\}_{s=1}^{t-1}$.
\end{assumption}

\paragraph{GP-UCB policy.}
Fix a nondecreasing sequence $\{\beta_t\}_{t\ge 1}$.
At round $t$, GP-UCB selects
\begin{equation}\label{eq:gp-ucb-policy}
x_t \in \argmax_{x\in\cX} \; \mu_{t-1}(x) + \sqrt{\beta_t}\,\sigma_{t-1}(x).
\end{equation}

\paragraph{Regret.}
Let $x^\star\in\argmax_{x\in\cX} f(x)$ be an optimal maximizer (assumed to exist).
Define the instantaneous and cumulative regret by
\begin{equation}\label{eq:regret-def}
r_t := f(x^\star)-f(x_t),\qquad
R_T := \sum_{t=1}^T r_t.
\end{equation}


\begin{lemma}[Uniform GP confidence bound]\label{lem:ucb-confidence}
Let $\delta\in(0,1)$ and let $\{\beta_t\}_{t\ge 1}$ be chosen such that, with probability at least $1-\delta$,
the event
\begin{equation}\label{eq:confidence-event}
\cE := \Big\{ \forall t\ge 1,\ \forall x\in\cX:\ |f(x)-\mu_{t-1}(x)| \le \sqrt{\beta_t}\,\sigma_{t-1}(x) \Big\}
\end{equation}
holds.
For example, if $\cX$ is finite, one may take
\begin{equation}\label{eq:beta-finite}
\beta_t \;=\; 2\log\!\Big(\frac{|\cX|\pi^2 t^2}{6\delta}\Big),
\end{equation}
which yields $\bbP(\cE)\ge 1-\delta$ by a Gaussian tail bound and a union bound over $x\in\cX$ and $t\ge 1$.
\end{lemma}

\begin{lemma}[Instantaneous regret is controlled by posterior uncertainty]\label{lem:instantaneous-regret}
On the event $\cE$ in \eqref{eq:confidence-event}, the GP-UCB action sequence \eqref{eq:gp-ucb-policy} satisfies
\begin{equation}\label{eq:rt-bound}
r_t \;\le\; 2\sqrt{\beta_t}\,\sigma_{t-1}(x_t)\qquad\text{for all }t\ge 1.
\end{equation}
\end{lemma}

\begin{proof}
Fix $t\ge 1$ and suppose $\cE$ holds.
By \eqref{eq:confidence-event},
\begin{equation}\label{eq:upper-fstar}
f(x^\star)\le \mu_{t-1}(x^\star)+\sqrt{\beta_t}\sigma_{t-1}(x^\star).
\end{equation}
Since $x_t$ maximizes the upper confidence bound in \eqref{eq:gp-ucb-policy},
\begin{equation}\label{eq:ucb-max}
\mu_{t-1}(x^\star)+\sqrt{\beta_t}\sigma_{t-1}(x^\star)
\le
\mu_{t-1}(x_t)+\sqrt{\beta_t}\sigma_{t-1}(x_t).
\end{equation}
Again by \eqref{eq:confidence-event},
\begin{equation}\label{eq:lower-ft}
f(x_t)\ge \mu_{t-1}(x_t)-\sqrt{\beta_t}\sigma_{t-1}(x_t).
\end{equation}
Combining \eqref{eq:upper-fstar}--\eqref{eq:lower-ft} yields
\[
r_t = f(x^\star)-f(x_t)
\le
\big(\mu_{t-1}(x_t)+\sqrt{\beta_t}\sigma_{t-1}(x_t)\big)
-
\big(\mu_{t-1}(x_t)-\sqrt{\beta_t}\sigma_{t-1}(x_t)\big)
=
2\sqrt{\beta_t}\sigma_{t-1}(x_t),
\]
which proves \eqref{eq:rt-bound}.
\end{proof}


\paragraph{Maximum information gain.}
For a set of query points $A=\{x_1,\dots,x_T\}\subset \cX$, let $f_A := (f(x))_{x\in A}$ and $y_A := (y(x))_{x\in A}$.
Define the \emph{maximum information gain} by
\begin{equation}\label{eq:gamma-def}
\gamma_T \;:=\; \max_{A\subset \cX,\ |A|=T} \I(y_A; f_A).
\end{equation}
In the Gaussian noise case, with kernel matrix $K_A \in \R^{T\times T}$ on $A$ and noise variance $\sigma^2$,
\begin{equation}\label{eq:mutual-info-gaussian}
\I(y_A;f_A) \;=\; \frac{1}{2}\log\det\!\big(I + \sigma^{-2}K_A\big).
\end{equation}

\begin{lemma}[Posterior variance sum is controlled by information gain]\label{lem:variance-sum}
Let $\{x_t\}_{t=1}^T$ be any sequence of query points and let $\sigma_{t-1}^2(x_t)$ be the GP posterior variance
at $x_t$ given data up to $t-1$.
Then there exists a constant $C_\sigma>0$ (depending only on the noise level) such that
\begin{equation}\label{eq:variance-sum}
\sum_{t=1}^T \sigma_{t-1}^2(x_t) \;\le\; C_\sigma\,\gamma_T.
\end{equation}
For instance, for homoscedastic Gaussian noise with variance $\sigma^2$ one may take
\begin{equation}\label{eq:Csigma}
C_\sigma \;=\; \frac{2}{\log(1+\sigma^{-2})},
\end{equation}
and \eqref{eq:variance-sum} holds (see, e.g., the GP-UCB analysis).
\end{lemma}


\begin{theorem}[GP-UCB regret bound]\label{thm:gp-ucb-regret}
Fix $\delta\in(0,1)$ and choose $\{\beta_t\}_{t\ge 1}$ such that the confidence event $\cE$ in
\eqref{eq:confidence-event} holds with probability at least $1-\delta$.
Assume $\beta_t$ is nondecreasing.
Then, with probability at least $1-\delta$, the cumulative regret of GP-UCB satisfies
\begin{equation}\label{eq:regret-main}
R_T \;\le\; 2\sqrt{C_\sigma\,T\,\beta_T\,\gamma_T}\qquad\text{for all }T\ge 1,
\end{equation}
where $\gamma_T$ is the maximum information gain in \eqref{eq:gamma-def} and $C_\sigma$ is as in
Lemma~\ref{lem:variance-sum}.
\end{theorem}

\begin{proof}
Work on the event $\cE$ (which holds w.p.\ $\ge 1-\delta$).
By Lemma~\ref{lem:instantaneous-regret} and monotonicity of $\beta_t$,
\begin{equation}\label{eq:rt-sum-step}
R_T = \sum_{t=1}^T r_t
\le
2\sum_{t=1}^T \sqrt{\beta_t}\,\sigma_{t-1}(x_t)
\le
2\sqrt{\beta_T}\sum_{t=1}^T \sigma_{t-1}(x_t).
\end{equation}
By Cauchy--Schwarz,
\begin{equation}\label{eq:cs}
\sum_{t=1}^T \sigma_{t-1}(x_t)
\le
\sqrt{T\sum_{t=1}^T \sigma_{t-1}^2(x_t)}.
\end{equation}
Combining \eqref{eq:rt-sum-step}--\eqref{eq:cs} and applying Lemma~\ref{lem:variance-sum} yields
\[
R_T
\le
2\sqrt{\beta_T}\sqrt{T\sum_{t=1}^T \sigma_{t-1}^2(x_t)}
\le
2\sqrt{\beta_T}\sqrt{T\cdot C_\sigma\,\gamma_T}
=
2\sqrt{C_\sigma\,T\,\beta_T\,\gamma_T},
\]
which proves \eqref{eq:regret-main}.
\end{proof}

\begin{remark}[Typical growth of $\gamma_T$]
For common kernels, $\gamma_T$ can be bounded as a function of $T$ and the input dimension $d$.
For example, for the squared-exponential (RBF) kernel on a compact subset of $\R^d$,
$\gamma_T = \tilde{\mathcal{O}}\big((\log T)^{d+1}\big)$, yielding sublinear regret
$R_T = \tilde{\mathcal{O}}\big(\sqrt{T}\,(\log T)^{(d+1)/2}\big)$ up to the growth of $\beta_T$.
\end{remark}

\subsubsection{Generalization to mixtures: loose max-k UCB}
 
\newcommand{\cF}{\mathcal{F}}

 
\begin{assumption}[Finite mixture of Gaussian processes]\label{ass:mogp}
Let $K\in\mathbb{N}$ and mixture weights $\pi_1,\dots,\pi_K$ satisfy $\pi_k>0$, $\sum_{k=1}^K \pi_k=1$.
A latent component index $z\in\{1,\dots,K\}$ is drawn as
\begin{equation}\label{eq:z-prior}
z \sim \mathrm{Categorical}(\pi_1,\dots,\pi_K).
\end{equation}
Conditioned on $z=k$, the unknown reward function $f:\cX\to\R$ is drawn from a GP prior
\begin{equation}\label{eq:gp-component}
f \mid (z=k) \sim \mathcal{GP}(0,\,k_k),
\end{equation}
with (known) covariance kernel $k_k$.
At each round $t\ge 1$, an algorithm chooses $x_t\in\cX$ and observes
\begin{equation}\label{eq:mogp-obs}
y_t = f(x_t) + \varepsilon_t,
\end{equation}
where $\{\varepsilon_t\}$ are conditionally $\sigma$-sub-Gaussian:
$\E[\exp(\lambda\varepsilon_t)\mid \cF_{t-1}] \le \exp(\tfrac12\sigma^2\lambda^2)$ for all $\lambda\in\R$,
and $\cF_{t-1}$ is the sigma-field generated by past $(x_s,y_s)_{s\le t-1}$.
\end{assumption}

\paragraph{Component posteriors.}
For each component $k\in\{1,\dots,K\}$, let $\mu_{t-1}^{(k)}(x)$ and $\sigma_{t-1}^{(k)}(x)$ denote the
GP posterior mean and standard deviation at $x\in\cX$ computed under the assumption $z=k$
using data $\{(x_s,y_s)\}_{s=1}^{t-1}$.
 
\paragraph{Regret.}
Let $x^\star\in\argmax_{x\in\cX} f(x)$ be an optimizer. Define
\begin{equation}\label{eq:mogp-regret}
r_t := f(x^\star)-f(x_t),\qquad R_T := \sum_{t=1}^T r_t.
\end{equation}
 
\paragraph{Robust MoGP-UCB.}
Fix nondecreasing sequences $\{\beta_t^{(k)}\}_{t\ge 1}$ for each component $k$.
Define the robust upper confidence bound
\begin{equation}\label{eq:robust-ucb}
U_t(x) \;:=\; \max_{k\in\{1,\dots,K\}}\Big\{ \mu_{t-1}^{(k)}(x) + \sqrt{\beta_t^{(k)}}\,\sigma_{t-1}^{(k)}(x)\Big\}.
\end{equation}
The MoGP-UCB action is
\begin{equation}\label{eq:mogp-ucb-policy}
x_t \in \argmax_{x\in\cX} U_t(x).
\end{equation}
 
\begin{lemma}[Uniform confidence tubes for all components]\label{lem:mogp-confidence}
Fix $\delta\in(0,1)$ and choose $\beta_t^{(k)}$ such that, with probability at least $1-\delta$,
the event
\begin{equation}\label{eq:mogp-E}
\mathcal{E} := \Big\{\forall t\ge 1,\ \forall x\in\cX,\ \forall k\in\{1,\dots,K\}:\ 
|f(x)-\mu_{t-1}^{(k)}(x)| \le \sqrt{\beta_t^{(k)}}\,\sigma_{t-1}^{(k)}(x)\Big\}
\end{equation}
holds.
For finite $\cX$ one convenient choice is
\begin{equation}\label{eq:beta-mogp-finite}
\beta_t^{(k)} \;=\; 2\log\!\Big(\frac{K\,|\cX|\,\pi^2 t^2}{6\delta}\Big),
\end{equation}
which yields $\bbP(\mathcal{E})\ge 1-\delta$ by a Gaussian tail bound and a union bound over $(t,x,k)$.
\end{lemma}
  
\begin{lemma}[Instantaneous regret under robust MoGP-UCB]\label{lem:mogp-instantaneous}
On the event $\mathcal{E}$ in \eqref{eq:mogp-E}, the robust MoGP-UCB policy \eqref{eq:mogp-ucb-policy} satisfies
\begin{equation}\label{eq:mogp-rt}
r_t \;\le\; 2\sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x_t)\qquad \text{for all }t\ge 1.
\end{equation}
\end{lemma}

\begin{proof}
Assume $\mathcal{E}$ holds and fix $t\ge 1$.
Using \eqref{eq:mogp-E} with the \emph{true} component $z$,
\begin{equation}\label{eq:mogp-upper-fstar}
f(x^\star)\le \mu_{t-1}^{(z)}(x^\star)+\sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x^\star).
\end{equation}
By definition of $U_t$ in \eqref{eq:robust-ucb},
\begin{equation}\label{eq:mogp-ucb-dominates}
\mu_{t-1}^{(z)}(x^\star)+\sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x^\star)
\le U_t(x^\star).
\end{equation}
Since $x_t$ maximizes $U_t(\cdot)$,
\begin{equation}\label{eq:mogp-max}
U_t(x^\star)\le U_t(x_t).
\end{equation}
Also, $U_t(x_t)\ge \mu_{t-1}^{(z)}(x_t)+\sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x_t)$ by the max over $k$.
Finally, again from \eqref{eq:mogp-E} with component $z$,
\begin{equation}\label{eq:mogp-lower-ft}
f(x_t)\ge \mu_{t-1}^{(z)}(x_t)-\sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x_t).
\end{equation}
Combining \eqref{eq:mogp-upper-fstar}--\eqref{eq:mogp-lower-ft} yields
\[
r_t = f(x^\star)-f(x_t)
\le
2\sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x_t),
\]
which proves \eqref{eq:mogp-rt}.
\end{proof}
 
\paragraph{Information gain for component $k$.}
For a set $A=\{x_1,\dots,x_T\}\subset\cX$, define
\begin{equation}\label{eq:gamma-k}
\gamma_T^{(k)} := \max_{A\subset\cX,\ |A|=T}\I\big(y_A;\ f_A \,\big|\, z=k\big).
\end{equation}
In the homoscedastic Gaussian noise case, with kernel matrix $K_A^{(k)}$,
\begin{equation}\label{eq:gamma-k-gaussian}
\I\big(y_A;\ f_A \,\big|\, z=k\big) = \frac12\log\det\!\big(I+\sigma^{-2}K_A^{(k)}\big).
\end{equation}

\begin{lemma}[Variance sum bound (component-wise)]\label{lem:mogp-variance-sum}
There exists a constant $C_\sigma>0$ (depending only on the noise level) such that for any query sequence
$\{x_t\}_{t=1}^T$ and any component $k$,
\begin{equation}\label{eq:mogp-variance-sum}
\sum_{t=1}^T \big(\sigma_{t-1}^{(k)}(x_t)\big)^2 \;\le\; C_\sigma\,\gamma_T^{(k)}.
\end{equation}
For homoscedastic Gaussian noise variance $\sigma^2$, one admissible choice is
$C_\sigma = 2/\log(1+\sigma^{-2})$.
\end{lemma}
 
\begin{theorem}[MoGP-UCB regret bound]\label{thm:mogp-regret}
Fix $\delta\in(0,1)$ and choose $\{\beta_t^{(k)}\}$ so that the uniform event $\mathcal{E}$ in \eqref{eq:mogp-E}
holds with probability at least $1-\delta$ (e.g.\ \eqref{eq:beta-mogp-finite} for finite $\cX$).
Assume each $\beta_t^{(k)}$ is nondecreasing in $t$.
Then, with probability at least $1-\delta$, the cumulative regret of robust MoGP-UCB satisfies
\begin{equation}\label{eq:mogp-main-regret}
R_T \;\le\; 2\sqrt{C_\sigma\,T\,\beta_T^{(z)}\,\gamma_T^{(z)}}\qquad\text{for all }T\ge 1,
\end{equation}
where $z$ is the (unknown) latent component generating $f$ and $\gamma_T^{(z)}$ is defined in \eqref{eq:gamma-k}.
In particular, a component-uniform (worst-case) bound is
\begin{equation}\label{eq:mogp-worstcase}
R_T \;\le\; 2\sqrt{C_\sigma\,T\,\Big(\max_{k}\beta_T^{(k)}\Big)\,\Big(\max_{k}\gamma_T^{(k)}\Big)}.
\end{equation}
\end{theorem}

\begin{proof}
Work on the event $\mathcal{E}$.
By Lemma~\ref{lem:mogp-instantaneous} and monotonicity of $\beta_t^{(z)}$,
\begin{align}
R_T
= \sum_{t=1}^T r_t
&\le 2\sum_{t=1}^T \sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x_t)
\le 2\sqrt{\beta_T^{(z)}}\sum_{t=1}^T \sigma_{t-1}^{(z)}(x_t).
\end{align}
Cauchy--Schwarz gives
\[
\sum_{t=1}^T \sigma_{t-1}^{(z)}(x_t)
\le \sqrt{T\sum_{t=1}^T \big(\sigma_{t-1}^{(z)}(x_t)\big)^2}.
\]
Apply Lemma~\ref{lem:mogp-variance-sum} with $k=z$ to obtain
\[
R_T \le 2\sqrt{\beta_T^{(z)}}\sqrt{T\cdot C_\sigma\,\gamma_T^{(z)}}
= 2\sqrt{C_\sigma\,T\,\beta_T^{(z)}\,\gamma_T^{(z)}}.
\]
The worst-case bound \eqref{eq:mogp-worstcase} follows immediately.
\end{proof}

\begin{remark}[Bayesian regret over the mixture]
Taking expectation w.r.t.\ $z\sim\mathrm{Categorical}(\pi)$,
\[
\E[R_T] \le 2\sqrt{C_\sigma\,T}\ \sum_{k=1}^K \pi_k \sqrt{\beta_T^{(k)}\,\gamma_T^{(k)}}
\le 2\sqrt{C_\sigma\,T}\ \sqrt{\sum_{k=1}^K \pi_k \beta_T^{(k)}\,\gamma_T^{(k)}},
\]
where the last inequality is Jensen (concavity of $\sqrt{\cdot}$).
\end{remark}

 

\newcommand{\KL}{\mathrm{KL}} 
\subsection{Generalization to mixtures: Moment-matched UCB}
 

\begin{assumption}[Mixture-of-GPs bandit model]\label{ass:mogp-mm}
Let $K\in\mathbb{N}$ and mixture weights $\pi_1,\dots,\pi_K$ satisfy $\pi_k>0$, $\sum_{k=1}^K \pi_k=1$.
A latent component index $z\in\{1,\dots,K\}$ is drawn as
\begin{equation}\label{eq:mm-z-prior}
z \sim \mathrm{Categorical}(\pi_1,\dots,\pi_K).
\end{equation}
Conditioned on $z=k$, the unknown reward function $f:\cX\to\R$ is drawn from a GP prior
\begin{equation}\label{eq:mm-gp-component}
f \mid (z=k) \sim \mathcal{GP}(0,\,k_k),
\end{equation}
with known kernel $k_k$. At each round $t\ge 1$, an algorithm chooses $x_t\in\cX$ and observes
\begin{equation}\label{eq:mm-obs}
y_t = f(x_t) + \varepsilon_t,
\end{equation}
where $\{\varepsilon_t\}$ are conditionally $\sigma$-sub-Gaussian:
$\E[\exp(\lambda\varepsilon_t)\mid \cF_{t-1}] \le \exp(\tfrac12\sigma^2\lambda^2)$ for all $\lambda\in\R$,
with $\cF_{t-1}$ generated by past $(x_s,y_s)_{s\le t-1}$.
\end{assumption}

\paragraph{Component posteriors.}
For each $k\in\{1,\dots,K\}$, let $\mu_{t-1}^{(k)}(x)$ and $\sigma_{t-1}^{(k)}(x)$ denote the GP posterior mean
and standard deviation at $x\in\cX$ computed under the conditional model $z=k$ using data
$\mathcal{D}_{t-1} := \{(x_s,y_s)\}_{s=1}^{t-1}$.
 
\paragraph{Posterior responsibilities.}
Let $w_{t-1}^{(k)} := \bbP(z=k \mid \mathcal{D}_{t-1})$.
By Bayes' rule,
\begin{equation}\label{eq:mm-resp}
w_{t-1}^{(k)}
=
\frac{\pi_k\,p(\mathcal{D}_{t-1}\mid z=k)}{\sum_{j=1}^K \pi_j\,p(\mathcal{D}_{t-1}\mid z=j)}.
\end{equation}
In the Gaussian noise case, $p(\mathcal{D}_{t-1}\mid z=k)$ is the standard GP marginal likelihood
(with kernel $k_k$ and noise variance $\sigma^2$).
 
\paragraph{Moment-matched predictive mean and variance.}
Let $\mathcal{D}_{t-1}$ be fixed. The exact predictive distribution of $f(x)$ under the mixture posterior is
\begin{equation}\label{eq:mm-mixture-posterior}
p\big(f(x)\mid \mathcal{D}_{t-1}\big)
=
\sum_{k=1}^K w_{t-1}^{(k)}\,
p\big(f(x)\mid \mathcal{D}_{t-1}, z=k\big),
\end{equation}
where $p(f(x)\mid \mathcal{D}_{t-1}, z=k)$ is Gaussian with mean $\mu_{t-1}^{(k)}(x)$ and variance
$(\sigma_{t-1}^{(k)}(x))^2$.

Define the moment-matched mean and variance by, see result in the main paper.
\begin{equation}\label{eq:mm-def-moments}
\mu_{t-1}^{\mathrm{mix}}(x) := \E\big[f(x)\mid \mathcal{D}_{t-1}\big],\qquad
\big(\sigma_{t-1}^{\mathrm{mix}}(x)\big)^2 := \Var\big(f(x)\mid \mathcal{D}_{t-1}\big).
\end{equation}

\paragraph{MM-MoGP-UCB policy.}
Fix a nondecreasing exploration sequence $\{\beta_t\}_{t\ge 1}$ and define
\begin{equation}\label{eq:mm-ucb}
U_t^{\mathrm{mix}}(x) := \mu_{t-1}^{\mathrm{mix}}(x) + \sqrt{\beta_t}\,\sigma_{t-1}^{\mathrm{mix}}(x).
\end{equation}
The moment-matched UCB action is
\begin{equation}\label{eq:mm-policy}
x_t \in \argmax_{x\in\cX} U_t^{\mathrm{mix}}(x).
\end{equation}

\paragraph{Regret.}
Let $x^\star\in\argmax_{x\in\cX} f(x)$ and define
\begin{equation}\label{eq:mm-regret}
r_t := f(x^\star)-f(x_t),\qquad R_T := \sum_{t=1}^T r_t.
\end{equation}
 
\begin{assumption}[Component-wise confidence tubes]\label{ass:mm-comp-tubes}
Fix $\delta\in(0,1)$ and choose (component-wise) $\{\beta_t^{(k)}\}_{t\ge 1}$ such that with probability at least
$1-\delta$,
\begin{equation}\label{eq:mm-comp-event}
\mathcal{E}_{\mathrm{comp}}
:=
\Big\{ \forall t\ge 1,\ \forall x\in\cX,\ \forall k\in\{1,\dots,K\}:\ 
|f(x)-\mu_{t-1}^{(k)}(x)| \le \sqrt{\beta_t^{(k)}}\,\sigma_{t-1}^{(k)}(x)\Big\}
\end{equation}
holds (e.g.\ for finite $\cX$ via a union bound over $(t,x,k)$).
\end{assumption}

\begin{assumption}[Lower bound on responsibility of the true component]\label{ass:mm-weight-lb}
There exists $\underline{w}\in(0,1]$ such that, for all $t\ge 1$,
\begin{equation}\label{eq:mm-weight-lb}
w_{t-1}^{(z)} = \bbP(z\mid \mathcal{D}_{t-1}) \ge \underline{w}.
\end{equation}
(For example, this can be enforced by truncating responsibilities away from $0$ in implementation,
or it may follow from additional identifiability/likelihood-ratio conditions.)
\end{assumption}

\begin{lemma}[Two deterministic inequalities linking $(\mu^{(z)},\sigma^{(z)})$ to $(\mu^{\mathrm{mix}},\sigma^{\mathrm{mix}})$]
\label{lem:mm-det-ineq}
Fix $t\ge 1$ and $x\in\cX$. Let $w:=w_{t-1}^{(z)}$.
Then
\begin{align}
\big(\sigma_{t-1}^{\mathrm{mix}}(x)\big)^2
&\ge
w\,\big(\sigma_{t-1}^{(z)}(x)\big)^2,
\label{eq:mm-sig-dom}\\
\big(\sigma_{t-1}^{\mathrm{mix}}(x)\big)^2
&\ge
w\,\big(\mu_{t-1}^{(z)}(x)-\mu_{t-1}^{\mathrm{mix}}(x)\big)^2.
\label{eq:mm-mean-gap-dom}
\end{align}
Consequently,
\begin{equation}\label{eq:mm-gap-bounds}
\sigma_{t-1}^{(z)}(x) \le \frac{1}{\sqrt{w}}\sigma_{t-1}^{\mathrm{mix}}(x),\qquad
\big|\mu_{t-1}^{(z)}(x)-\mu_{t-1}^{\mathrm{mix}}(x)\big|\le \frac{1}{\sqrt{w}}\sigma_{t-1}^{\mathrm{mix}}(x).
\end{equation}
\end{lemma}

\begin{proof}
From \eqref{eq:mm-var}, since all terms are nonnegative and $w_{t-1}^{(z)}=w$,
\[
\big(\sigma_{t-1}^{\mathrm{mix}}(x)\big)^2
=
\sum_{k=1}^K w_{t-1}^{(k)}\Big((\sigma_{t-1}^{(k)}(x))^2 + (\mu_{t-1}^{(k)}(x)-\mu_{t-1}^{\mathrm{mix}}(x))^2\Big)
\ge
w\,(\sigma_{t-1}^{(z)}(x))^2,
\]
proving \eqref{eq:mm-sig-dom}. Dropping the within-component variance terms instead yields
\[
\big(\sigma_{t-1}^{\mathrm{mix}}(x)\big)^2 \ge w\,(\mu_{t-1}^{(z)}(x)-\mu_{t-1}^{\mathrm{mix}}(x))^2,
\]
proving \eqref{eq:mm-mean-gap-dom}. Taking square roots gives \eqref{eq:mm-gap-bounds}.
\end{proof}

\begin{lemma}[Sufficient confidence tube for the moment-matched moments]\label{lem:mm-mix-confidence}
Assume $\mathcal{E}_{\mathrm{comp}}$ holds. Then for all $t\ge 1$ and $x\in\cX$,
\begin{equation}\label{eq:mm-mix-tube-pre}
|f(x)-\mu_{t-1}^{\mathrm{mix}}(x)|
\le
\left(\frac{\sqrt{\beta_t^{(z)}}+1}{\sqrt{w_{t-1}^{(z)}}}\right)\sigma_{t-1}^{\mathrm{mix}}(x).
\end{equation}
Under Assumption~\ref{ass:mm-weight-lb}, i.e.\ $w_{t-1}^{(z)}\ge \underline{w}$, the uniform tube
\begin{equation}\label{eq:mm-mix-tube}
|f(x)-\mu_{t-1}^{\mathrm{mix}}(x)| \le \sqrt{\beta_t}\,\sigma_{t-1}^{\mathrm{mix}}(x)
\qquad\text{for all }t\ge 1,\ x\in\cX
\end{equation}
holds with
\begin{equation}\label{eq:mm-beta-choice}
\beta_t := \frac{\big(\sqrt{\beta_t^{\max}}+1\big)^2}{\underline{w}},
\qquad \beta_t^{\max} := \max_{k\in\{1,\dots,K\}}\beta_t^{(k)}.
\end{equation}
\end{lemma}

\begin{proof}
Fix $t,x$ and write $w:=w_{t-1}^{(z)}$.
By the triangle inequality,
\begin{equation}\label{eq:mm-tri}
|f(x)-\mu_{t-1}^{\mathrm{mix}}(x)|
\le
|f(x)-\mu_{t-1}^{(z)}(x)|
+
|\mu_{t-1}^{(z)}(x)-\mu_{t-1}^{\mathrm{mix}}(x)|.
\end{equation}
On $\mathcal{E}_{\mathrm{comp}}$, the first term is bounded by $\sqrt{\beta_t^{(z)}}\,\sigma_{t-1}^{(z)}(x)$.
Apply \eqref{eq:mm-gap-bounds} to both terms:
\[
|f(x)-\mu_{t-1}^{\mathrm{mix}}(x)|
\le
\sqrt{\beta_t^{(z)}}\frac{1}{\sqrt{w}}\sigma_{t-1}^{\mathrm{mix}}(x)
+
\frac{1}{\sqrt{w}}\sigma_{t-1}^{\mathrm{mix}}(x)
=
\left(\frac{\sqrt{\beta_t^{(z)}}+1}{\sqrt{w}}\right)\sigma_{t-1}^{\mathrm{mix}}(x),
\]
proving \eqref{eq:mm-mix-tube-pre}. Under $w\ge \underline{w}$ and $\beta_t^{(z)}\le \beta_t^{\max}$,
\[
\left(\frac{\sqrt{\beta_t^{(z)}}+1}{\sqrt{w}}\right)^2
\le
\frac{(\sqrt{\beta_t^{\max}}+1)^2}{\underline{w}}=\beta_t,
\]
which yields \eqref{eq:mm-mix-tube}.
\end{proof}
 
\begin{lemma}[Instantaneous regret for MM-MoGP-UCB]\label{lem:mm-inst-regret}
Assume the moment-matched tube \eqref{eq:mm-mix-tube} holds (e.g.\ by Lemma~\ref{lem:mm-mix-confidence}).
Then the MM-MoGP-UCB policy \eqref{eq:mm-policy} satisfies
\begin{equation}\label{eq:mm-rt}
r_t \le 2\sqrt{\beta_t}\,\sigma_{t-1}^{\mathrm{mix}}(x_t)\qquad\text{for all }t\ge 1.
\end{equation}
\end{lemma}

\begin{proof}
Identical to the standard GP-UCB proof: on \eqref{eq:mm-mix-tube},
\[
f(x^\star)\le \mu_{t-1}^{\mathrm{mix}}(x^\star)+\sqrt{\beta_t}\sigma_{t-1}^{\mathrm{mix}}(x^\star)
\le
\mu_{t-1}^{\mathrm{mix}}(x_t)+\sqrt{\beta_t}\sigma_{t-1}^{\mathrm{mix}}(x_t),
\]
and also $f(x_t)\ge \mu_{t-1}^{\mathrm{mix}}(x_t)-\sqrt{\beta_t}\sigma_{t-1}^{\mathrm{mix}}(x_t)$,
which together imply \eqref{eq:mm-rt}.
\end{proof}
 
\paragraph{A variance-sum control for moment-matched uncertainty.}
The standard GP-UCB regret proof closes by bounding $\sum_{t\le T}\sigma_{t-1}^2(x_t)$ via information gain.
For the moment-matched mixture variance $\big(\sigma_{t-1}^{\mathrm{mix}}(\cdot)\big)^2$, the posterior is
not Gaussian; thus one typically assumes or proves an analogue of the variance-sum lemma.

\begin{assumption}[Variance-sum bound for moment-matched uncertainty]\label{ass:mm-varsum}
There exist a functional $\gamma_T^{\mathrm{mix}}$ (interpretable as a complexity / information-gain term for the
moment-matched model) and a constant $C_\sigma>0$ such that for any query sequence $\{x_t\}_{t=1}^T$,
\begin{equation}\label{eq:mm-varsum}
\sum_{t=1}^T \big(\sigma_{t-1}^{\mathrm{mix}}(x_t)\big)^2 \le C_\sigma\,\gamma_T^{\mathrm{mix}}.
\end{equation}
\end{assumption}

\begin{theorem}[MM-MoGP-UCB regret bound (template)]\label{thm:mm-regret}
Fix $\delta\in(0,1)$ and suppose Assumptions~\ref{ass:mm-comp-tubes} and \ref{ass:mm-weight-lb} hold,
so that the moment-matched tube \eqref{eq:mm-mix-tube} holds with probability at least $1-\delta$
(e.g.\ via Lemma~\ref{lem:mm-mix-confidence} and a union bound for $\mathcal{E}_{\mathrm{comp}}$).
Assume $\beta_t$ is nondecreasing and Assumption~\ref{ass:mm-varsum} holds.
Then with probability at least $1-\delta$, the cumulative regret of MM-MoGP-UCB satisfies
\begin{equation}\label{eq:mm-main-regret}
R_T \le 2\sqrt{C_\sigma\,T\,\beta_T\,\gamma_T^{\mathrm{mix}}}\qquad \text{for all }T\ge 1.
\end{equation}
\end{theorem}

\begin{proof}
On the tube \eqref{eq:mm-mix-tube}, Lemma~\ref{lem:mm-inst-regret} yields
\[
R_T \le 2\sum_{t=1}^T \sqrt{\beta_t}\,\sigma_{t-1}^{\mathrm{mix}}(x_t)
\le 2\sqrt{\beta_T}\sum_{t=1}^T \sigma_{t-1}^{\mathrm{mix}}(x_t).
\]
Cauchy--Schwarz gives $\sum_{t=1}^T \sigma_{t-1}^{\mathrm{mix}}(x_t)\le
\sqrt{T\sum_{t=1}^T(\sigma_{t-1}^{\mathrm{mix}}(x_t))^2}$, and Assumption~\ref{ass:mm-varsum} closes the bound.
\end{proof}

 


% \newpage

% \section{***DRAFT OUTLINE*** Proof of regret bound and convergence}
% %
% Our theoretical result shows that the convergence of ordinary GP-EI is conditionally inherited by RAMBO.
% The proof follows a two-part strategy. First, we use a well-known result from the literature and show that it directly applies cluster-wise, i.e. based on the cluster marginal likelihood. In a second step, we infer the mixture regret bound and convergence through cluster-wise conditioning on the DP.
% %
% %
% %\subsection{Tran The path}
% %
% We start with Theorem 1 in \cite{tran-the2022}, which provides convergence guarantees for EI with a modified exploration parameter. This modification  is crucial for the proof to hold for noisy BO. For noise-less BO, this part of the proof simplifies significantly and we can instead use  \emph{ordinary} EI based on results by \cite{bull2011convergence}. However, our novelty is the synthesis of the known strategies for GPs with a cluster-wise DP argument, rather than a specific setting and corresponding strategy for a single GP alone. As such, the settings and strategies are exchangeable and we limit ourselves do demonstrating it for noisy BO with modified EI. 
 
% Let
% %
% \[
% x^\star \in \arg\max_{x\in\mathcal X} f(x)
% \]
% %
% denote a global maximizer of the unknown function $f$.
% The cumulative regret after $T$ iterations is defined as
% %
% \begin{equation} \label{eq:def-cumulative-regret}
% R_T
% \;:=\;
% \sum_{t=1}^T \bigl( f(x^\star) - f(x_t) \bigr).
% \end{equation}
% %
% Now consider the following modified EI acquisition function,
% %
% \begin{equation} \label{eq:modified-EI}
% \alpha_{t,\Omega}^{\mathrm{EI}}(x)
% =
% \bigl(\mu_{t-1}(x)-\mu_t^+\bigr)
% \Phi\!\left(
% \frac{\mu_{t-1}(x)-\mu_t^+}{\Omega_t\,\sigma_{t-1}(x)}
% \right)
% +
% \Omega_t\,\sigma_{t-1}(x)\,
% \phi\!\left(
% \frac{\mu_{t-1}(x)-\mu_t^+}{\Omega_t\,\sigma_{t-1}(x)}
% \right),
% \end{equation}
% %
% with $\Omega_t = \sqrt{\gamma_{t-1} + 1 + \ln\!\left(\tfrac{1}{\delta}\right)}$, wherein $\gamma_t := \max_{A \subset \mathcal X,\ |A| = t} I\!\left( y_A ; f_A \right)$ is the maximum information gain at time $t$. 
% %where $\Omega_t =1 \forall t$ restores ordinary EI.

% Then Theorem 1 in \cite{tran-the2022} is
% %
% \begin{theorem}
%     Let $\delta \in (0,1)$. Then with probability at least $1-\delta$, the cumulative regret \eqref{eq:def-cumulative-regret} for the EI acquisition function $\alpha_{t,\Omega}^{\mathrm{EI}}(x)$ \eqref{eq:modified-EI} is bounded as
%     \begin{equation}
%         R_T = \mathcal{O}(\gamma_T \sqrt{T})
%     \end{equation}
% \end{theorem}
% %
% Since the gating weights $w_k(\mathbf{x}_*) \approx p(z_* = k \mid \mathbf{x}_*, \mathcal{D})$ with regime weights \eqref{eq:regime_weights} $	w_k(\mathbf{x}_*) \propto \frac{n_k}{n + \alpha} \cdot \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right)$.
% %

% %
% Now introduce the conditional EI as $\mathbb{E}[\max(0, f(x)-f^+) \mid z_\ast =k ] = \alpha_{k, t,\Omega}^{\mathrm{EI}}(x)$. In other words, the mixture EI conditioned on the assignment $z$ is merely the ordinary EI with the single GP (cluster) $k$ that is being conditioned on.
% We can condition Theorem D.1. on the regime, i.e. for the conditional EI we restore
% %
% \begin{align}
%     P\big((R_T \leq \mathcal{O}(\gamma_T \sqrt{T}) \mid z_\ast =k\big) \geq 1-\delta
% \end{align}
% %
% Then 
% %
% \begin{align}
%     P\big((R_T \leq \mathcal{O}(\gamma_T \sqrt{T})) &= \sum_k P\big((R_T \leq \mathcal{O}(\gamma_T \sqrt{T}) \mid z_\ast =k\big)\cdot \frac{n_k}{n + \alpha} \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right) \\
%     % &\leq (1-\delta) K \max_k \frac{n_k}{n + \alpha} \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right) \\
%     % &\leq (1-\delta) K (n+\alpha)   \max_k  \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right) 
%     &\geq (1-\delta) \sum_k \frac{n_k}{n + \alpha} \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right)\\ 
%     &\geq  \frac{1-\delta}{n + \alpha}\sum_k \exp\left(-\frac{1}{2}\log \sigma^2_{*,k}(\mathbf{x}_*)\right)\\ 
% \end{align}
% %
% since $n_k \geq 1$.

% Now consider the modified conditional DPMM-GP-EI
% %
% \begin{align}
% \text{EI}^{(\Omega)}_{\text{DPMM}}(\mathbf{x}) &= \sum_{k=1}^{K} w_k(\mathbf{x}) \;  \alpha_{t,k}^{\mathrm{EI}}(x) \\
% &\leq K\cdot \max_k \big( w_k(\mathbf{x}) \; \alpha_{t,k}^{\mathrm{EI}}(x) \big)
% \end{align}

% \subsection{Auxiliary reminders}

% The Cluster Marginal Likelihood \eqref{prop:marginal} is $p(\mathbf{y}_k \mid \mathbf{X}_k, \theta_k) = \mathcal{N}(\mathbf{y}_k \mid \mathbf{0}, \mathbf{K}_k + \sigma^2_{n,k}\mathbf{I})$.


% \begin{equation}
% \text{EI}_{\text{DPMM}}(\mathbf{x}) = \sum_{k=1}^{K} w_k(\mathbf{x}) \cdot \sigma_{*,k}(\mathbf{x}) [\gamma_k \Phi(\gamma_k) + \phi(\gamma_k)]
% \end{equation}

%  \begin{theorem}[Cumulative Regret Bound]
% Let $f \sim \mathcal{GP}(0, k)$ with $\|f\|_k \leq B$. Using DPMM-GP-UCB with $\beta_t = 2B^2 + 300\gamma_t\log^3(t/\delta)$:
% \begin{equation}
% R_T = \sum_{t=1}^T (f(\mathbf{x}^*) - f(\mathbf{x}_t)) = O(\sqrt{T\gamma_T \log T})
% \end{equation}
% with probability at least $1-\delta$, where $\gamma_T$ is the maximum information gain.
% \end{theorem}






% %%%%%%%%%


% \subsection{Bull path}
% %
% \begin{theorem}[Bull, 2011 --- Convergence rate of Expected Improvement]
% Let $\mathcal X \subset \mathbb{R}^d$ be compact with non-empty interior, and let
% $\pi$ be a Gaussian process prior with covariance kernel $K_\theta$.
% Denote by $\mathcal H_\theta(\mathcal X)$ the associated reproducing-kernel Hilbert space.

% For a strategy $u$, define the simple regret after $n$ evaluations by
% \[
% L_n(u,\mathcal H_\theta(\mathcal X),R)
% :=
% \sup_{\|f\|_{\mathcal H_\theta(\mathcal X)} \le R}
% \mathbb E_f\!\left[f(x_n^\star)-\min_{x\in\mathcal X} f(x)\right],
% \]
% where $x_n^\star$ is the best point observed up to time $n$.
% Assume the kernel $K_\theta$ satisfies Assumptions~1--4 of \cite{Bull2011},
% with smoothness parameter $\nu>0$ and logarithmic exponent $\alpha \ge 0$.
% Then the Expected Improvement strategy with fixed prior $\pi$ satisfies
% \[
% L_n(\mathrm{EI}(\pi),\mathcal H_\theta(\mathcal X),R)
% =
% \begin{cases}
% O\!\left(n^{-\nu/d}(\log n)^{\alpha}\right), & \nu \le 1,\\[6pt]
% O\!\left(n^{-1/d}\right), & \nu > 1.
% \end{cases}
% \]
% \end{theorem}


==> sections/suppl_sascha.tex <==
\section{MES}

\subsection{Max-value Entropy Search (MES)}

We further extend the DPMM-GP to entropy-based search. Max-value Entropy Search (MES) seeks to maximize the mutual information between the candidate observation $y$ at $\mathbf{x}$ and the global maximum value $y^* = \max_{\mathbf{x}' \in \mathcal{X}} f(\mathbf{x}')$. The acquisition function is defined as:
\begin{equation}
	\alpha_{\text{MES}}(\mathbf{x}) = H(y \mid \mathbf{x}) - \mathbb{E}_{y^*} \left[ H(y \mid \mathbf{x}, y < y^*) \right].
\end{equation}

For the DPMM-GP, the first term $H(y \mid \mathbf{x})$ is the entropy of the predictive mixture derived in Theorem \ref{thm:predictive}. While the entropy of a Gaussian mixture has no closed form, we approximate it via the entropy of a single Gaussian with moment-matched variance $\sigma^2_{\text{mix}}(\mathbf{x})$:
\begin{equation}
	H(y \mid \mathbf{x}) \approx \frac{1}{2} \log(2\pi e \sigma^2_{\text{mix}}(\mathbf{x})).
\end{equation}

For the second term, we estimate the expectation over $y^*$ via Monte Carlo sampling. We sample $y^*_s \sim p(y^*)$ by first sampling a regime $k \sim \boldsymbol{\pi}$ and then sampling the maximum of that GP component (e.g., via Gumbel approximation). Given a sample $y^*_s$, the conditional entropy is computed using the truncated Gaussian approximation for each component weighted by $w_k(\mathbf{x})$:
\begin{equation}
	\mathbb{E}_{y^*} [H(\dots)] \approx \frac{1}{S} \sum_{s=1}^S \sum_{k=1}^K w_k(\mathbf{x}) \left[ \frac{\gamma_{k,s} \phi(\gamma_{k,s})}{2\Phi(\gamma_{k,s})} - \ln \Phi(\gamma_{k,s}) \right],
\end{equation}
where $\gamma_{k,s} = (y^*_s - \mu_{*,k}(\mathbf{x})) / \sigma_{*,k}(\mathbf{x})$. This formulation directs sampling toward regions that maximally reduce uncertainty about the global maximum across all latent regimes.

\newpage

\section{Complete Optimization Loop of \ours}

\ours integrates the DPMM-GP surrogate with a sequential acquisition strategy. The complete procedure is outlined in Algorithm \ref{alg:bo_loop} and proceeds through four distinct phases at each iteration $t$:

\begin{enumerate}
	\item \textbf{Initialization:} We initialize the procedure with a small seed dataset $\mathcal{D}_0$ generated via Latin Hypercube Sampling (LHS) to ensuring a space-filling coverage of the domain $\mathcal{X}$ before the model guides the search.
	
	\item \textbf{Inference with Warm Starts:} To reduce the computational burden of MCMC, we employ a \textit{warm start} strategy. Instead of re-initializing the sampler from scratch, we initialize the Gibbs sampler (Algorithm \ref{alg:gibbs}) using the assignments $\mathbf{z}^{(t-1)}$ and hyperparameters $\Theta^{(t-1)}$ from the previous iteration. This significantly reduces the burn-in period required to reach the stationary distribution.
	
	\item \textbf{Acquisition Optimization:} We maximize the mixture Expected Improvement $\alpha_{\text{EI}}(\mathbf{x})$. Since the acquisition landscape is inherently multimodal (inheriting local optima from multiple regime-specific GPs), we optimize it using a multi-start L-BFGS-B approach. The optimizer is initialized with a hybrid set of candidates $\mathcal{S}_{init}$ comprising: (1) uniform random samples, (2) centroids of currently active regimes, and (3) local perturbations of the current best solution $\mathbf{x}^*$.
	
	\item \textbf{Feedback and Maintenance:} After evaluating the selected candidate $\mathbf{x}_{new}$, we augment the dataset and perform a maintenance step. We prune any ``dead'' regimes (empty clusters or weights $\pi_k < \epsilon$) to maintain a compact model representation and prevent unnecessary computation in subsequent matrix inversions.
\end{enumerate}

\begin{algorithm}[h]
	\caption{DPMM-GP Bayesian Optimization Loop}
	\label{alg:bo_loop}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} Search space $\mathcal{X}$, budget $T_{\text{max}}$, initial size $n_{\text{init}}$
		\STATE {\bfseries Parameters:} MCMC samples $S$, restarts $R$, prune threshold $\epsilon$
		\STATE {\bfseries Output:} Best solution $\mathbf{x}^*$
		
		\STATE \textit{// Phase 1: Initialization}
		\STATE $\mathcal{D}_0 \leftarrow$ LatinHypercubeSampling($\mathcal{X}, n_{\text{init}}$)
		\STATE Initialize $\Theta^{(0)}$ and $\mathbf{z}^{(0)}$ randomly
		\STATE $\mathbf{x}^* \leftarrow \text{argmax}_{(\mathbf{x},y) \in \mathcal{D}_0} y$
		
		\FOR{$t = 1$ {\bfseries to} $T_{\text{max}}$}
		\STATE \textit{// Phase 2: Inference (Warm Start)}
		\STATE Run Collapsed Gibbs (Alg. \ref{alg:gibbs}) for $S$ steps initialized with $(\Theta^{(t-1)}, \mathbf{z}^{(t-1)})$
		\STATE Collect posterior samples $\{\Theta^{(s)}, \mathbf{z}^{(s)}\}_{s=1}^S$
		\STATE Compute mixture moments $\mu_{\text{mix}}(\mathbf{x}), \sigma_{\text{mix}}(\mathbf{x})$ and weights $w_k(\mathbf{x})$ (Thm. \ref{thm:mixture_stats})
		
		\STATE \textit{// Phase 3: Acquisition Optimization}
		\STATE Define $\alpha_{\text{EI}}(\mathbf{x})$ per Eq. \eqref{eq:ei_dpmm}
		\STATE Generate start points $\mathcal{S}_{init} \leftarrow \{ \text{Uniform}(\mathcal{X}) \} \cup \{ \text{Centroids}(\mathbf{z}) \} \cup \{ \mathbf{x}^* + \delta \}$
		\STATE $\mathbf{x}_{new} \leftarrow \text{argmax}_{\mathbf{x} \in \mathcal{S}_{init}} \text{L-BFGS-B}(\alpha_{\text{EI}}(\mathbf{x}))$
		
		\STATE \textit{// Phase 4: Evaluation \& Update}
		\STATE $y_{new} \leftarrow f(\mathbf{x}_{new}) + \varepsilon$
		\STATE $\mathcal{D}_t \leftarrow \mathcal{D}_{t-1} \cup \{(\mathbf{x}_{new}, y_{new})\}$
		\IF{$y_{new} > f(\mathbf{x}^*)$}
		\STATE $\mathbf{x}^* \leftarrow \mathbf{x}_{new}$
		\ENDIF
		
		\STATE \textit{// Phase 5: Maintenance}
		\STATE Update $(\Theta^{(t)}, \mathbf{z}^{(t)})$ using the last MCMC sample
		\STATE Prune regimes where $\sum_i \mathbb{I}(z_i = k) < 1$ or $\pi_k < \epsilon$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\newpage

%\section{Adaptive Concentration Parameter Scheduling}
%\label{sec:alpha_scheduling}
%
%The concentration parameter $\alpha$ governs the model's propensity to instantiate new latent regimes. Standard approaches treat $\alpha$ as a fixed hyperparameter or infer it via a static prior. We argue that for sequential optimization, the \emph{optimal} model complexity is non-stationary. We propose an \textbf{adaptive $\alpha$-scheduling} mechanism that dynamically adjusts the prior to match the rate of information gain.
%
%\subsection{Motivation: The Regime Discovery Dilemma}
%The optimal value of $\alpha$ depends on the optimization phase:
%\begin{itemize}
%	\item \textbf{Exploration (Early Stage):} Regime inference is highly uncertain. A large $\alpha$ encourages fragmentation, creating sparse regimes with insufficient data for robust GP hyperparameter estimation. Conversely, a negligible $\alpha$ forces heterogeneous data into a single stationary GP. A moderate $\alpha$ is required to balance parsimony with flexibility.
%	\item \textbf{Discovery (Middle Stage):} As observations accumulate, the latent structure becomes discernible. Increasing $\alpha$ allows the model to capture finer-grained heterogeneity, isolating distinct basins of attraction into separate regimes with locally adapted length scales.
%	\item \textbf{Exploitation (Late Stage):} As $n \to \infty$, a fixed $\alpha$ in a standard DP implies that the probability of forming a new cluster decays as $\mathcal{O}(1/n)$. However, in complex multi-modal landscapes, we may continue to encounter new basins. The schedule must counteract the ``rich-get-richer'' dynamic of the Chinese Restaurant Process to maintain sensitivity to novel structures.
%\end{itemize}
%
%\subsection{Theoretical Foundation}
%We formalize the scheduling by matching the prior's expected complexity to a target discovery rate.
%
%\begin{proposition}
%	\label{prop:alpha_scaling}
%	Assume the number of discernible regimes $K^*$ grows with sample size $n$ at a polynomial rate $\mathcal{O}(n^\beta)$ (e.g., $\beta=0.5$ for square-root growth). To align the Dirichlet Process prior expectation $\mathbb{E}[K_n \mid \alpha]$ with this rate, the concentration parameter must scale as:
%	\begin{equation}
%		\alpha^*(n) \propto \frac{n^\beta}{\log n}
%		\label{eq:optimal_alpha}
%	\end{equation}
%\end{proposition}
%\noindent The derivation is provided in Appendix~\ref{app:alpha_proof}. This scaling ensures that the model capacity grows sufficiently to accommodate new regimes without overfitting.
%
%\subsection{Proposed Strategy: Log-Sqrt Schedule}
%Guided by Proposition~\ref{prop:alpha_scaling} with $\beta=1/2$, we employ the \textit{Log-Sqrt Schedule}:
%\begin{equation}
%	\alpha_t = \alpha_0 \cdot \frac{\sqrt{t}}{\log(t+e)}
%\end{equation}
%where $\alpha_0$ is a base concentration (default 1.0). This schedule aligns with the ``Square Root Rule'' often used in clustering heuristics, ensuring a balance between exploration (regime formation) and exploitation (regime consolidation) throughout the optimization budget.
%
%\subsection{Derivation of the Log-Sqrt Scaling Law}
%\label{app:alpha_proof}
%
%In this section, we derive the optimal scaling for the concentration parameter $\alpha$ to achieve a desired growth rate in the number of latent regimes.
%
%\subsection{Expected Number of Regimes}
%Under the Chinese Restaurant Process (CRP) representation of the Dirichlet Process, the expected number of distinct clusters (regimes) $K_n$ observed after $n$ samples, given a concentration parameter $\alpha$, is given exactly by:
%\begin{equation}
%	\mathbb{E}[K_n \mid \alpha] = \sum_{i=1}^n \frac{\alpha}{\alpha + i - 1}
%\end{equation}
%For $n \gg 1$ and fixed $\alpha$, this sum is well-approximated by \cite{antoniak1974mixtures}:
%\begin{equation}
%	\mathbb{E}[K_n \mid \alpha] \approx \alpha \log\left(1 + \frac{n}{\alpha}\right)
%	\label{eq:antoniak}
%\end{equation}
%
%\subsection{Target Growth Rate}
%Standard DP mixtures assume logarithmic cluster growth ($K_n \sim \alpha \log n$), which effectively assumes a ``rich-get-richer'' phenomenon where new structures become exponentially harder to find. In global optimization over multi-modal landscapes, we assume the discovery of distinct basins of attraction follows a power law relation with the number of samples, analogous to Heap's Law in information retrieval or the ``Square Root Rule'' in clustering.[1] We set our target growth rate as:
%\begin{equation}
%	K^*(n) \propto n^\beta \quad \text{where } \beta \in (0, 1)
%\end{equation}
%For the Log-Sqrt schedule, we select $\beta = 1/2$.
%
%\subsection{Asymptotic Derivation}
%We seek a time-dependent schedule $\alpha_n$ such that $\mathbb{E}[K_n \mid \alpha_n] \asymp n^\beta$. Substituting the approximation from Eq.~\eqref{eq:antoniak}:
%\begin{equation}
%	\alpha_n \log\left(1 + \frac{n}{\alpha_n}\right) \asymp n^\beta
%\end{equation}
%Let us hypothesize a scaling of the form $\alpha_n = c \frac{n^\beta}{\log n}$ for some constant $c$. Substituting this into the LHS:
%\begin{align}
%	\text{LHS} &= c \frac{n^\beta}{\log n} \log\left(1 + \frac{n}{c \frac{n^\beta}{\log n}}\right) \\
%	&= c \frac{n^\beta}{\log n} \log\left(1 + \frac{n^{1-\beta} \log n}{c}\right)
%\end{align}
%Considering the limit as $n \to \infty$:
%\begin{enumerate}
%	\item The term inside the logarithm is dominated by $n^{1-\beta}$.
%	\item We can approximate $\log(1 + x) \approx \log(x)$ for large $x$.
%\end{enumerate}
%
%\begin{equation}
%	\text{LHS} \approx c \frac{n^\beta}{\log n} \log\left(\frac{n^{1-\beta} \log n}{c}\right)
%\end{equation}
%Expanding the logarithm:
%\begin{equation}
%	\text{LHS} \approx c \frac{n^\beta}{\log n} \left[ (1-\beta)\log n + \log(\log n) - \log c \right]
%\end{equation}
%Dominated by the leading term $(1-\beta)\log n$:
%\begin{equation}
%	\text{LHS} \approx c \frac{n^\beta}{\log n} \cdot (1-\beta)\log n = c(1-\beta) n^\beta
%\end{equation}
%Thus, $\mathbb{E}[K_n \mid \alpha_n]$ scales as $\mathcal{O}(n^\beta)$.
%
%\textbf{Conclusion:} To achieve a square-root growth rate ($\beta=1/2$) in the number of regimes, the concentration parameter must scale as:
%\begin{equation}
%	\alpha_n \propto \frac{\sqrt{n}}{\log n}
%\end{equation}
%This confirms that the Log-Sqrt schedule $\alpha_t = \alpha_0 \frac{\sqrt{t}}{\log t}$ provides the necessary prior flexibility to support polynomial regime discovery rates.


